Cerberus: A Blockchain-Based Accreditation and Degree Verification System

Credential fraud is a widespread practice that undermines investment and confidence in higher education systems and bears significant economic and social costs. Legacy credential verification systems are typically time-consuming, costly, and bureaucratic, and struggle against certain classes of credential fraud. In this paper, we propose a comprehensive blockchain-based credential verification solution, Cerberus, which is considerably more efficient, easy and intuitive to use, and effectively mitigates widespread manifestations of credential fraud. Cerberus also improves significantly upon other blockchain-based solutions in the research literature: it adheres closely to the existing credential verification ecosystem, it addresses a threat model informed by real-world fraud scenarios. Moreover, Cerberus uses on-chain smart contracts for credential revocation, and it does not entail students or employers to manage digital identities or cryptographic credentials to use the system. We prototype our solution and describe our attempt to design an online verification service with a rich feature set, including data privacy, transcript verification, and selective disclosure of data. We hope this effort contributes positively to towards alleviating the problem of fake credentials.

==> Contracts.tex <==
\begin{figure*}

\begin{minipage}{0.48\textwidth}
\begin{mdframed}  
\setlength{\parindent}{5ex}

\noindent {\fontfamily{qhv}\selectfont Contract Rules Engine}

\noindent \newline
\noindent  \textbf{Inputs:} {\fontfamily{qhv}\selectfont A${}_{n}$$\mathrm{\{}$$\mathrm{\}}$}

\noindent \textbf{Revoking Authority-List (A${}_{n}$):}

\noindent On receiving (A)

\noindent \textbf{if} 
{\fontfamily{qhv}\selectfont( E.address \textbf{$\boldsymbol{\mathrm{\in }}$ }A${}_{n}$$\mathrm{\{}$$\mathrm{\}}$):

\emph{A${}_{n}$$\{$$\}$ := A U A${}_{n}$$\{$$\}$}}

\noindent \textbf{else}
\newline
\indent {\fontfamily{qhv}\selectfont A $\in $ An$\{$$\}$ , has x 2 public keys}

\noindent \textbf{Rules (A.address):}

\noindent \textbf{if} 
{\fontfamily{qhv}\selectfont( A \textbf{$\boldsymbol{\mathrm{\in }}$} A${}_{n}$$\mathrm{\{}$$\mathrm{\}}$ \& A has not previously revoked the same document):

\indent Revoke count := Revoke count ++

\emph{return (true)}}

\noindent \textbf{else} 
\newline \indent {\fontfamily{qhv}\selectfont {Revoke count := Revoke count}}

%\newline

\noindent \newline A${}_{n}$$\mathrm{\{}$$\mathrm{\}}$ = Revoking Authority-List

\noindent A = Revoking Authority

\noindent E = any Entity in the Ecosystem

\end{mdframed}
\caption{Rules Engine}
\label{fig:revrules}
\end{minipage}\hfill
\end{figure*}

\begin{figure*}
\begin{minipage}{0.48\textwidth}
\begin{mdframed}
\setlength{\parindent}{5ex}

\noindent {\fontfamily{qhv}\selectfont
\noindent Contract Implementation Engine\textbf{ }}
\noindent \newline

\noindent \textbf{Inputs:} {\fontfamily{qhv}\selectfont D${}_{H}$, P${}_{H}$}

\noindent {\fontfamily{qhv}\selectfont \noindent r = Rules Engine (adressRulesEngine)}

\noindent \textbf{Revoke Document (D${}_{H}$):}

\noindent {\fontfamily{qhv}\selectfont \emph{call r.Rules (A.address)}}

\noindent \textbf{if} {\fontfamily{qhv}\selectfont (r.Rules (A.address)=true): 
\newline \indent \emph{return (PH)}}

\noindent \textbf{else}

\indent {\fontfamily{qhv}\selectfont \emph{terminate process}}

\noindent \textbf{Confirm Revocation (P${}_{H}$):}

\noindent {\fontfamily{qhv}\selectfont \emph{call r.Rules (A.address)}}

\noindent \textbf{if}
{\fontfamily{qhv}\selectfont (r.Rules (A.address)=true \& Revoke count = requiredCount):}
\newline \indent {\fontfamily{qhv}\selectfont \emph{call Revoke List (DH)}}

\noindent \textbf{else} 
\newline \indent {\fontfamily{qhv}\selectfont \emph{terminate process}}

\noindent \textbf{Revoke-List (D${}_{H}$):}

\noindent {\fontfamily{qhv}\selectfont Revoke-List$\mathrm{\{}$$\mathrm{\}}$ := D${}_{H\ }$U Revoke List$\mathrm{\{}$$\mathrm{\}}$}

\noindent \textbf{Output:} {\fontfamily{qhv}\selectfont {''PH'', Revoke-List}}

\noindent \newline
\noindent D${}_{H}$ = Hash of Document
\noindent P${}_{H}$ = Process Hash
\noindent requiredCount = revocation count required for successful revocation
\end{mdframed}
\caption{Implementation Engine}
    \label{fig:revcredential}
\end{minipage}
\end{figure*}



==> notes.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[htbp]
  \centering
  \caption{Features Comparison}
    \begin{tabular}{p{5.93em}p{5.57em}p{5.93em}p{3.355em}p{3.215em}p{4.285em}p{6em}p{4.645em}p{5em}p{4.645em}}
    \toprule
    \textbf{Scheme} & \multicolumn{3}{p{14.855em}}{\textbf{Scope}} & \multicolumn{6}{p{27.79em}|}{\textbf{System Model}} \\
    \midrule
    \multicolumn{1}{|c}{} & \textit{\textbf{Target}} & \textit{\textbf{Institutions\newline{}Involved}} & \textit{\textbf{Bound}} & \multicolumn{6}{p{27.79em}|}{\textit{\textbf{Core \newline{}Mechanism}}} \\
    \midrule
    \multicolumn{1}{|r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{c}{\textit{Type}} & \multicolumn{1}{c}{\textit{Platform}} & \multicolumn{1}{c}{\textit{Issuance}} & \multicolumn{1}{c}{\textit{Verification}} & \textit{Verification Input} & \multicolumn{1}{c|}{\textit{Revocation}} \\
    \midrule
    \textbf{Legacy} & Academic Credentials & Accreditation Authority, University & Nation wide & -     & Paper Based  & Paper Based & Manual Application  & Original Academic Credential & Paper Based \\
    \midrule
    \textbf{UNIC \cite{nicosia}} & UNIC Certificates & UNIC  & UNIC  & Public & Bitcoin & OP-RETURN field in an unspendable transaction & Lookup & PDF of Certificate & - \\
    \midrule
    \textbf{Blockcerts \cite{blockcerts}} & Civic records, Academic credentials, professional licenses, etc. & -     & -     & Public & Bitcoin, Ethereum & OP-RETURN field in an unspendable transaction & Lookup &  Mozilla Open Badges (JSON or PDF) & Issuer-hosted revocation list \\
    \midrule
    \textbf{Echo \cite{echo}} & Academic Credentials, Career Details & -     & Echo Users  & Public & Ethereum, AntShares, Metaverseetc & Smart contracts  & Search by attributes & Search by attributes & - \\
    \midrule
    \textbf{UZHBC \cite{uzhbc}} & UZH Diplomas & UZHBC & UZHBC & Public &  Ethereum & Smart contracts  & Smart contracts  & PDF of Certificate & - \\
    \midrule
    \textbf{EduCtx \cite{EduCTX}} & Higher Education credit and Grading & European Credit Transfer and Accumulation System (ECTS) & Global & Private & Ark   & Transferring tokens to Students Blockchain address &  Blockchain address and redeem script &  Blockchain address and redeem script & - \\
    \midrule
    \textbf{Blockchain for Education \cite{bc4edu}} & Academic Credentials & Accreditation Authority, University & Global & Public &  Ethereum & Smart Contracts  & Smart Contracts  &  Mozilla Open Badges (JSON or PDF) & Smart Contracts  \\
    \midrule
    \textbf{Cerberus} & Academic Credentials & Accreditation Authority, University & Nation wide & Private &  Parity (Ethereum Client) & Batch Issuance Transaction & Lookup & QR Code & Rule Based Multi Party Smart Contracts  \\
    \bottomrule
    \end{tabular}%
  \label{tab:featurescomparison}%
\end{table*}%



